Adversarial Networks and Autoencoders: The Primal-Dual Relationship and Generalization Bounds

Since the introduction of Generative Adversarial Networks (GANs) and Variational Autoencoders (VAE), the literature on generative modelling has witnessed an overwhelming resurgence. The impressive, yet elusive empirical performance of GANs has lead to the rise of many GAN-VAE hybrids, with the hopes of GAN level performance and additional benefits of VAE, such as an encoder for feature reduction, which is not offered by GANs. Recently, the Wasserstein Autoencoder (WAE) was proposed, achieving performance similar to that of GANs, yet it is still unclear whether the two are fundamentally different or can be further improved into a unified model. In this work, we study the $f$-GAN and WAE models and make two main discoveries. First, we find that the $f$-GAN and WAE objectives partake in a primal-dual relationship and are equivalent under some assumptions, which then allows us to explicate the success of WAE. Second, the equivalence result allows us to, for the first time, prove generalization bounds for Autoencoder models, which is a pertinent problem when it comes to theoretical analyses of generative models. Furthermore, we show that the WAE objective is related to other statistical quantities such as the $f$-divergence and in particular, upper bounded by the Wasserstein distance, which then allows us to tap into existing efficient (regularized) optimal transport solvers. Our findings thus present the first primal-dual relationship between GANs and Autoencoder models, comment on generalization abilities and make a step towards unifying these models.

==> content/conclusion.tex <==
\section{Conclusion}
Our generalization bounds hold for discrete distributions and make a suitable scenario for computational methods that typically make such assumptions. Finally, we explored the effect of weighting the reconstruction and regularization, showing relationships to both $f$-divergences and Wasserstein metrics. variations of $f$-WAE under different costs and $f$, showing that it is related to $f$-divergences and in particular the entropy regularized Wasserstein distance. This allows us to use efficient solvers to minimize $f$-WAE, generalization bounds and by equivalence, $f$-GANs. Future work will include studying the case when the set of encoders class is restricted, and a result relating some notion of the complexity of a restricted encoder class to generalization. Other lines of future work can include considering costs $c$ that are not metrics and using the general dual of the Wasserstein distance to formulate a GAN.


==> content/pushforward.tex <==
\section{Partial Pushforwards}
In this section, we define a notion of a partial pushforward, which relaxes the moment constraint.
\begin{definition}($\mathcal{F}$-Pushforward)
Let $\mathcal{F} \subseteq \mathscr{F}(\mathcal{X},\mathbb{R})$ and consider two distributions $P,Q \in \mathscr{P}(\mathcal{X})$, a function $T: \mathcal{X} \to \mathcal{X}$ is said to $\mathcal{F}$-Pushforward $P$ to $Q$ if \begin{align} \forall f \in \mathcal{F} : \E_{x \sim P}[f(T(x))] = \E_{x \sim Q}[f(x)].\end{align} 
\end{definition}
It should be noted that when $\mathcal{F}$ is taken to be all measurable functions, then the $\mathcal{F}$-Pushforward corresponds to the standard pushforward and so the capacity of $\mathcal{F}$ can be associated with the capability of being a pushforward. We now outline some properties of a partial pushforward that demonstrate its use in determining capacity.
\begin{lemma}
\label{properties-of-partial-pushforwards}
Let $P,Q \in \mathscr{P}(\mathcal{X})$,  $\mathcal{F} \subseteq \mathscr{F}(\mathcal{X}, \mathbb{R})$ and $T$ be a $\mathcal{F}$-Pushforward from $P$ to $Q$ then we have 
\begin{enumerate}
	\item (Monotonicty) For any $\mathcal{F'} \subseteq \mathcal{F}$, $T$ is a $\mathcal{F'}$-Pushforward from $P$ to $Q$.
	\item (Dense) If $P$ and $Q$ are discrete and suppose there exists $\mathcal{H}$ such that $\mathcal{F}$ is dense in $\mathcal{H}$ then $T$ is a $\mathcal{H}$-Pushforward from $P$ to $Q$.
	\item (Convex Hulls) $T$ is a $\text{co}\bracket{\mathcal{F}}$-Pushforward from $P$ to $Q$.
	\item (Inverses) If a function $H$ is a right inverse of $T$ then $H$ is a $\bracket{\mathcal{F} \circ T}$-Pushforward from $Q$ to $P$.
\end{enumerate}
\end{lemma}
